An Empirical Study of Fault Localization in Python Programs

Despite its massive popularity as a programming language, especially in novel domains like data science programs, there is comparatively little research about fault localization that targets Python. Even though it is plausible that several findings about programming languages like C/C++ and Java -- the most common choices for fault localization research -- carry over to other languages, whether the dynamic nature of Python and how the language is used in practice affect the capabilities of classic fault localization approaches remain open questions to investigate. This paper is the first multi-family large-scale empirical study of fault localization on real-world Python programs and faults. Using Zou et al.'s recent large-scale empirical study of fault localization in Java as the basis of our study, we investigated the effectiveness (i.e., localization accuracy), efficiency (i.e., runtime performance), and other features (e.g., different entity granularities) of seven well-known fault-localization techniques in four families (spectrum-based, mutation-based, predicate switching, and stack-trace based) on 135 faults from 13 open-source Python projects from the BugsInPy curated collection. The results replicate for Python several results known about Java, and shed light on whether Python's peculiarities affect the capabilities of fault localization. The replication package that accompanies this paper includes detailed data about our experiments, as well as the tool FauxPy that we implemented to conduct the study.

==> data-example.tex <==
\pgfkeyssetvalue{/flpy/num projects}{4}
\pgfkeyssetvalue{/flpy/statement/einspect/sbfl/keras/5}{12.5}
\pgfkeyssetvalue{/flpy/statement/einspect/sbfl/keras/7}{1.436545}
\pgfkeyssetvalue{/flpy/statement/einspect/pvalue}{1.66433659543306e-02}
\pgfkeyssetvalue{/flpy/project:4}{Keras}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

% 


==> data.tex <==
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/time}{-1}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/einspect}{66}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/@1}{53}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/@3}{71}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/@5}{76}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/@10}{84}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/exam}{0.0720454802458773}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/javaexam}{0.013006330013549632}
\pgfkeyssetvalue{/flpy/func/avfl/alfa/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/time}{-1}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/einspect}{66}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/@1}{44}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/@3}{64}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/@5}{73}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/@10}{79}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/exam}{0.07414000002690645}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/javaexam}{0.015268411377061086}
\pgfkeyssetvalue{/flpy/func/avfl/sbst/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/time}{-1}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/einspect}{66}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/@1}{48}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/@3}{67}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/@5}{74}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/@10}{82}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/exam}{0.07309274013639187}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/javaexam}{0.014137370695305358}
\pgfkeyssetvalue{/flpy/func/avfl/favg/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/time}{589}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/einspect}{67}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/@1}{36}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/@3}{61}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/@5}{71}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/@10}{78}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/exam}{0.07434851496984929}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/javaexam}{0.015648646275129314}
\pgfkeyssetvalue{/flpy/func/sbfl/tarantula/all/outputlength}{296.31111111111113}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/time}{589}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/einspect}{67}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/@1}{38}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/@3}{61}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/@5}{72}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/@10}{79}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/exam}{0.07429098916267678}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/javaexam}{0.015586518403382993}
\pgfkeyssetvalue{/flpy/func/sbfl/ochiai/all/outputlength}{296.31111111111113}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/time}{589}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/einspect}{67}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/@1}{37}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/@3}{61}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/@5}{72}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/@10}{79}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/exam}{0.0742769463179623}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/javaexam}{0.01557135213109137}
\pgfkeyssetvalue{/flpy/func/sbfl/dstar/all/outputlength}{296.31111111111113}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/time}{15774}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/einspect}{93}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/@1}{34}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/@3}{56}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/@5}{64}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/@10}{70}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/exam}{0.11440468766666244}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/javaexam}{0.013497065802816822}
\pgfkeyssetvalue{/flpy/func/mbfl/metallaxis/all/outputlength}{30.666666666666668}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/time}{15774}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/einspect}{97}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/@1}{27}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/@3}{46}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/@5}{57}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/@10}{64}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/exam}{0.11691600104235392}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/javaexam}{0.016579132218438226}
\pgfkeyssetvalue{/flpy/func/mbfl/muse/all/outputlength}{30.666666666666668}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/time}{9751}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/einspect}{618}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/@1}{8}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/@3}{13}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/@5}{13}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/@10}{15}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/exam}{0.4047228068308939}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/javaexam}{0.002537295786867146}
\pgfkeyssetvalue{/flpy/func/ps/favg/all/outputlength}{0.562962962962963}
\pgfkeyssetvalue{/flpy/func/st/favg/all/time}{2}
\pgfkeyssetvalue{/flpy/func/st/favg/all/einspect}{451}
\pgfkeyssetvalue{/flpy/func/st/favg/all/@1}{21}
\pgfkeyssetvalue{/flpy/func/st/favg/all/@3}{27}
\pgfkeyssetvalue{/flpy/func/st/favg/all/@5}{27}
\pgfkeyssetvalue{/flpy/func/st/favg/all/@10}{29}
\pgfkeyssetvalue{/flpy/func/st/favg/all/exam}{0.3375483217008306}
\pgfkeyssetvalue{/flpy/func/st/favg/all/javaexam}{0.00448981826856575}
\pgfkeyssetvalue{/flpy/func/st/favg/all/outputlength}{0.9925925925925926}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/time}{589}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/einspect}{67}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/@1}{37}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/@3}{61}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/@5}{72}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/@10}{79}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/exam}{0.07430548348349612}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/javaexam}{0.015602172269867891}
\pgfkeyssetvalue{/flpy/func/sbfl/favg/all/outputlength}{296.31111111111113}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/time}{15774}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/einspect}{95}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/@1}{31}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/@3}{51}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/@5}{61}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/@10}{67}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/exam}{0.11566034435450817}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/javaexam}{0.015038099010627524}
\pgfkeyssetvalue{/flpy/func/mbfl/favg/all/outputlength}{30.666666666666668}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/time}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/einspect}{2356}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/@3}{42}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/@5}{60}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/@10}{74}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/exam}{0.05749241780411741}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/javaexam}{0.005648677113810365}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/outputlength}{687.1162790697674}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/cli/distance}{5.1047232499089805}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/time}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/einspect}{2356}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/@3}{42}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/@5}{60}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/@10}{74}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/exam}{0.05745867350106107}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/javaexam}{0.00561049277087819}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/outputlength}{687.1162790697674}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/cli/distance}{5.3186060766626975}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/time}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/einspect}{2356}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/@3}{42}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/@5}{60}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/@10}{74}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/exam}{0.05745867350106107}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/javaexam}{0.00561049277087819}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/outputlength}{687.1162790697674}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/cli/distance}{5.3186060766626975}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/time}{3770}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/einspect}{2909}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/@3}{30}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/@5}{35}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/@10}{44}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/exam}{0.17595006401716312}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/javaexam}{0.0031892887239549244}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/outputlength}{34.27906976744186}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/cli/distance}{22.788008401814235}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/time}{3770}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/einspect}{2912}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/@5}{42}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/@10}{47}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/exam}{0.17599488073180183}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/javaexam}{0.003266373473133597}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/outputlength}{34.27906976744186}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/cli/distance}{5.668161380293332}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/time}{528}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/einspect}{8667}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/@1}{2}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/@3}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/@5}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/@10}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/exam}{0.29720957961531863}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/javaexam}{0.0002078437110832702}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/outputlength}{0.3023255813953488}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/cli/distance}{10.035731386409157}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/einspect}{9124}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/@3}{9}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/@5}{9}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/@10}{14}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/exam}{0.2675176621450724}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/javaexam}{0.00837604832542256}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/outputlength}{19.930232558139537}
\pgfkeyssetvalue{/flpy/stmt/st/favg/cli/distance}{8.503424399789266}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/time}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/einspect}{2356}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/@3}{42}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/@5}{60}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/@10}{74}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/exam}{0.057469921602079845}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/javaexam}{0.005623220885188914}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/outputlength}{687.1162790697675}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/cli/distance}{5.2473118010781254}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/time}{3770}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/einspect}{2910}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/@1}{9}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/@5}{38}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/@10}{45}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/exam}{0.1759724723744825}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/javaexam}{0.003227831098544261}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/outputlength}{34.27906976744186}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/cli/distance}{14.228084891053783}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/time}{589}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/@1}{59}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/@3}{84}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/@5}{91}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/exam}{0.042215430678112266}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/javaexam}{0.037501269388558946}
\pgfkeyssetvalue{/flpy/mod/sbfl/tarantula/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/time}{589}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/@1}{61}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/@3}{87}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/exam}{0.04124790565790988}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/javaexam}{0.0365265240323849}
\pgfkeyssetvalue{/flpy/mod/sbfl/ochiai/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/time}{589}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/@1}{61}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/@3}{87}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/exam}{0.04126264935606302}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/javaexam}{0.03654137775813619}
\pgfkeyssetvalue{/flpy/mod/sbfl/dstar/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/time}{15774}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/einspect}{6}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/@1}{57}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/@3}{82}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/@5}{87}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/@10}{92}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/exam}{0.07248257070689533}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/javaexam}{0.03660543125938902}
\pgfkeyssetvalue{/flpy/mod/mbfl/metallaxis/all/outputlength}{5.57037037037037}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/time}{15774}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/einspect}{7}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/@1}{47}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/@3}{77}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/@5}{85}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/@10}{87}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/exam}{0.07991533022926521}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/javaexam}{0.04463281154354846}
\pgfkeyssetvalue{/flpy/mod/mbfl/muse/all/outputlength}{5.57037037037037}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/time}{9751}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/einspect}{67}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/@1}{13}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/@3}{17}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/@5}{21}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/@10}{28}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/exam}{0.41634670834970977}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/javaexam}{0.023441892101774497}
\pgfkeyssetvalue{/flpy/mod/ps/favg/all/outputlength}{0.3925925925925926}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/time}{2}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/einspect}{61}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/@1}{29}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/@3}{33}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/@5}{36}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/@10}{41}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/exam}{0.33632876193476285}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/javaexam}{0.02838005830515854}
\pgfkeyssetvalue{/flpy/mod/st/favg/all/outputlength}{0.5851851851851851}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/time}{589}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/@1}{60}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/@3}{86}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/@5}{92}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/exam}{0.041575328564028395}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/javaexam}{0.036856390393026676}
\pgfkeyssetvalue{/flpy/mod/sbfl/favg/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/time}{15774}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/einspect}{6}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/@1}{52}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/@3}{80}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/@5}{86}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/@10}{90}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/exam}{0.07619895046808027}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/javaexam}{0.04061912140146874}
\pgfkeyssetvalue{/flpy/mod/mbfl/favg/all/outputlength}{5.57037037037037}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/time}{1284}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/einspect}{377}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/@3}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/@5}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/@10}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/exam}{0.015396784507531578}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/javaexam}{0.006521340740361081}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/outputlength}{3041.5384615384614}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/pred/distance}{12.67360960552377}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/time}{1284}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/einspect}{372}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/@3}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/@5}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/@10}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/exam}{0.015360611475504677}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/javaexam}{0.006483720787053104}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/outputlength}{3041.5384615384614}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/pred/distance}{13.207893594627036}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/time}{1284}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/einspect}{371}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/@3}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/@5}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/@10}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/exam}{0.015352218336156572}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/javaexam}{0.006474991922131078}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/outputlength}{3041.5384615384614}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/pred/distance}{13.583468767178802}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/time}{19671}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/einspect}{1882}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/@3}{37}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/@5}{44}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/@10}{56}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/exam}{0.028250016562632544}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/javaexam}{0.003773762189448894}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/outputlength}{146.46153846153845}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/pred/distance}{26.362795517508136}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/time}{19671}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/einspect}{1899}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/@1}{10}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/@3}{29}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/@5}{37}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/@10}{48}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/exam}{0.02715994157640326}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/javaexam}{0.0025141199831394965}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/outputlength}{146.46153846153845}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/pred/distance}{32.61515162106886}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/time}{17287}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/einspect}{8425}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/@1}{8}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/@3}{13}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/@5}{17}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/@10}{17}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/exam}{0.14929941753331805}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/javaexam}{0.00010556862466765817}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/outputlength}{1.25}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/pred/distance}{12.335695507867522}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/einspect}{9194}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/@3}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/@5}{6}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/@10}{17}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/exam}{0.15410411274276103}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/javaexam}{0.0007208885632961376}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/outputlength}{47.15384615384615}
\pgfkeyssetvalue{/flpy/stmt/st/favg/pred/distance}{7.438756894266723}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/time}{1284}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/einspect}{374}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/@3}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/@5}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/@10}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/exam}{0.015369871439730945}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/javaexam}{0.006493351149848421}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/outputlength}{3041.5384615384614}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/pred/distance}{13.154990655776537}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/time}{19671}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/einspect}{1891}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/@1}{11}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/@10}{52}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/exam}{0.027704979069517903}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/javaexam}{0.0031439410862941952}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/outputlength}{146.46153846153845}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/pred/distance}{29.488973569288497}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/time}{-1}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/einspect}{1575}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/@1}{18}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/@3}{36}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/@5}{47}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/@10}{59}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/exam}{0.05128261837553908}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/javaexam}{0.003302528846968437}
\pgfkeyssetvalue{/flpy/stmt/avfl/alfa/all/outputlength}{2548.362962962963}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/time}{-1}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/einspect}{1585}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/@5}{44}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/@10}{56}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/exam}{0.051863927447538566}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/javaexam}{0.0039583916263026715}
\pgfkeyssetvalue{/flpy/stmt/avfl/sbst/all/outputlength}{2548.3333333333335}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/time}{-1}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/einspect}{1580}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/@1}{15}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/@5}{46}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/@10}{57}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/exam}{0.05157327291153882}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/javaexam}{0.0036304602366355543}
\pgfkeyssetvalue{/flpy/stmt/avfl/favg/all/outputlength}{2548.3481481481485}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/time}{1726}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/einspect}{833}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/@1}{7}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/@3}{24}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/@5}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/@10}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/exam}{0.006802047086120662}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/javaexam}{0.001852224252099376}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/outputlength}{5775.357142857143}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/ds/distance}{15.29586728769396}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/time}{1726}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/einspect}{825}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/@1}{7}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/@3}{24}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/@5}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/@10}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/exam}{0.006733464769448151}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/javaexam}{0.0017819691959958285}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/outputlength}{5775.357142857143}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/ds/distance}{16.028889219116973}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/time}{1726}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/einspect}{824}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/@1}{5}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/@3}{21}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/@5}{29}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/@10}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/exam}{0.006728664395308205}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/javaexam}{0.0017770517395597854}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/outputlength}{5775.357142857143}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/ds/distance}{16.931973281172787}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/time}{29799}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/einspect}{14507}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/@1}{7}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/@3}{17}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/@5}{21}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/@10}{26}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/exam}{0.1721599625176657}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/javaexam}{0.0002519834799297213}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/outputlength}{169.28571428571428}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/ds/distance}{37.81426957020117}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/time}{29799}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/einspect}{14530}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/@3}{7}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/@5}{17}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/@10}{21}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/exam}{0.17247685694574405}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/javaexam}{0.0008857723360864847}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/outputlength}{169.28571428571428}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/ds/distance}{50.54031784669837}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/time}{15972}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/einspect}{22847}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/@1}{2}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/@3}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/@5}{7}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/@10}{7}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/exam}{0.27861196417079476}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/javaexam}{2.3971379930046436e-05}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/outputlength}{1.0}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/ds/distance}{18.320865667796674}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/einspect}{15174}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/@3}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/@5}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/@10}{12}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/exam}{0.17226288044301047}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/javaexam}{0.0003469045961527693}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/outputlength}{97.69047619047619}
\pgfkeyssetvalue{/flpy/stmt/st/favg/ds/distance}{8.173656907497048}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/time}{1726}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/einspect}{827}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/@1}{6}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/@3}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/@5}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/@10}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/exam}{0.006754725416959006}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/javaexam}{0.0018037483958849966}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/outputlength}{5775.357142857142}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/ds/distance}{16.085576595994574}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/time}{29799}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/einspect}{14519}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/@1}{4}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/@3}{12}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/@5}{19}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/@10}{24}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/exam}{0.17231840973170487}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/javaexam}{0.0005688779080081029}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/outputlength}{169.28571428571428}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/ds/distance}{44.17729370844977}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/time}{589}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/einspect}{1586}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/@3}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/@10}{54}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/exam}{0.051662620778257194}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/javaexam}{0.004189992725541162}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/outputlength}{2521.348148148148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/all/distance}{10.310770590103361}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/time}{589}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/einspect}{1583}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@3}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@10}{54}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/exam}{0.05163232006860066}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/javaexam}{0.004155904427177535}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/outputlength}{2521.348148148148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/distance}{10.616494823874216}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/time}{589}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/einspect}{1583}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@1}{11}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@3}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@5}{42}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@10}{54}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/exam}{0.051630826618868225}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/javaexam}{0.0041542242962285545}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/outputlength}{2521.348148148148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/distance}{10.897454309847138}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/time}{15774}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/einspect}{6706}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@1}{10}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@3}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@5}{30}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@10}{37}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/exam}{0.17256415741554368}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/javaexam}{0.003470449924030685}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/outputlength}{113.8962962962963}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/distance}{32.12070167204071}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/time}{15774}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/einspect}{6714}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@1}{6}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@3}{19}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@5}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@10}{32}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/exam}{0.17194447287313444}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/javaexam}{0.0023244579620409615}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/outputlength}{113.8962962962963}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/distance}{22.90044297241492}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/time}{9751}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/einspect}{11945}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@1}{3}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@3}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@5}{7}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@10}{7}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/exam}{0.2787497218988966}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/javaexam}{0.00010556862466765817}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/outputlength}{1.0296296296296297}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/distance}{17.116777563553907}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/einspect}{9810}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@3}{4}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@5}{6}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@10}{13}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/exam}{0.2241291127567302}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/javaexam}{0.002402072293431907}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/outputlength}{42.85925925925926}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/distance}{8.243865648880641}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/time}{589}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/einspect}{1584}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/@3}{30}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/@10}{54}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/exam}{0.05164192248857536}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/javaexam}{0.0041667071496490835}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/outputlength}{2521.348148148148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/all/distance}{10.608239907941572}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/time}{15774}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/einspect}{6710}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/@1}{8}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/@3}{22}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/@5}{27}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/@10}{34}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/exam}{0.17225431514433906}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/javaexam}{0.0028974539430358234}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/outputlength}{113.8962962962963}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/all/distance}{27.510572322227816}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/time}{231}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/einspect}{770}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/@1}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/@3}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/@10}{45}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/exam}{0.12359384557041267}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/javaexam}{0.0048632250404120865}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/outputlength}{1266.35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/web/distance}{12.720402450413863}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/time}{231}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/einspect}{770}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/@1}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/@3}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/@10}{45}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/exam}{0.1236051424524732}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/javaexam}{0.004879363443355731}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/outputlength}{1266.35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/web/distance}{12.770402450413863}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/time}{231}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/einspect}{770}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/@1}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/@3}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/@10}{45}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/exam}{0.1236051424524732}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/javaexam}{0.004879363443355731}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/outputlength}{1266.35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/web/distance}{12.770402450413863}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/time}{7753}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/einspect}{1469}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/@1}{10}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/@3}{20}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/@5}{20}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/@10}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/exam}{0.21270208692968975}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/javaexam}{0.004927144409854644}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/outputlength}{98.65}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/web/distance}{39.80167049619566}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/time}{7753}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/einspect}{1460}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/@1}{5}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/@3}{15}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/@5}{20}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/@10}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/exam}{0.21214506830792698}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/javaexam}{0.0035345978554476515}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/outputlength}{98.65}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/web/distance}{15.337936969627435}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/time}{828}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/einspect}{2362}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/@1}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/@3}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/@5}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/@10}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/exam}{0.274473269502389}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/javaexam}{0.00022716946842344388}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/outputlength}{1.05}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/web/distance}{20.308287272828476}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/time}{1}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/einspect}{2319}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/@3}{5}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/@5}{5}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/@10}{15}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/exam}{0.2631058856251216}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/javaexam}{0.0014071383509049152}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/outputlength}{22.65}
\pgfkeyssetvalue{/flpy/stmt/st/favg/web/distance}{8.70625}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/time}{231}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/einspect}{770}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/@1}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/@3}{15}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/@10}{45}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/exam}{0.1236013768251197}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/javaexam}{0.00487398397570785}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/outputlength}{1266.35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/web/distance}{12.753735783747196}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/time}{7753}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/einspect}{1465}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/@1}{8}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/@3}{18}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/@5}{20}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/@10}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/exam}{0.21242357761880837}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/javaexam}{0.004230871132651148}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/outputlength}{98.65}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/web/distance}{27.56980373291155}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/time}{890}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/einspect}{903}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/@1}{14}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/@3}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/@10}{53}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/exam}{0.04662088093730834}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/javaexam}{0.00254115899205032}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/outputlength}{3147.469387755102}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/crash/distance}{11.688373677354202}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/time}{890}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/einspect}{895}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/@1}{14}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/@3}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/@10}{53}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/exam}{0.04656670706671579}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/javaexam}{0.002480828999799537}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/outputlength}{3147.469387755102}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/crash/distance}{12.337086353267805}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/time}{890}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/einspect}{894}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/@1}{14}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/@3}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/@10}{53}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/exam}{0.04655780006169332}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/javaexam}{0.0024709098351154164}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/outputlength}{3147.469387755102}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/crash/distance}{12.735655924139065}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/time}{18278}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/einspect}{7793}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/@3}{29}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/@5}{33}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/@10}{37}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/exam}{0.16728461318059687}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/javaexam}{0.0008556603018041637}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/outputlength}{104.40816326530613}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/crash/distance}{42.69853431266601}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/time}{18278}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/einspect}{7818}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/@1}{2}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/@3}{14}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/@5}{20}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/@10}{31}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/exam}{0.1682339412771017}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/javaexam}{0.0026447786375248315}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/outputlength}{104.40816326530613}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/crash/distance}{43.09180646796559}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/time}{11419}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/einspect}{15607}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/@3}{0}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/@5}{0}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/@10}{0}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/exam}{0.29940246505546325}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/javaexam}{None}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/outputlength}{0.30612244897959184}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/crash/distance}{13.835314811282768}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/einspect}{5273}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/@3}{10}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/@5}{16}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/@10}{37}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/exam}{0.09286682401942466}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/javaexam}{0.002402072293431907}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/outputlength}{118.08163265306122}
\pgfkeyssetvalue{/flpy/stmt/st/favg/crash/distance}{5.161670665283396}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/time}{890}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/einspect}{897}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/@1}{14}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/@3}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/@5}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/@10}{53}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/exam}{0.04658179602190582}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/javaexam}{0.0024976326089884244}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/outputlength}{3147.469387755102}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/crash/distance}{12.253705318253692}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/time}{18278}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/einspect}{7806}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/@1}{7}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/@3}{21}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/@5}{27}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/@10}{34}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/exam}{0.16775927722884929}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/javaexam}{0.0017502194696644977}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/outputlength}{104.40816326530613}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/crash/distance}{42.8951703903158}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/time}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/einspect}{2081}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/@1}{20}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/@5}{37}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/@10}{47}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/exam}{0.05815723168207835}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/javaexam}{0.005337890808826007}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/outputlength}{1431.4666666666667}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/dev/distance}{9.187215160881484}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/time}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/einspect}{2081}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/@1}{20}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/@5}{37}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/@10}{47}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/exam}{0.05815772931163908}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/javaexam}{0.005338443730560148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/outputlength}{1431.4666666666667}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/dev/distance}{9.196844790511113}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/time}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/einspect}{2081}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/@1}{20}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/@5}{37}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/@10}{47}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/exam}{0.05815772931163908}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/javaexam}{0.005338443730560148}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/outputlength}{1431.4666666666667}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/dev/distance}{9.196844790511113}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/time}{18694}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/einspect}{4718}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/@1}{13}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/@5}{40}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/@10}{50}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/exam}{0.14151827780082132}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/javaexam}{0.006784306210421347}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/outputlength}{160.63333333333333}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/dev/distance}{32.40592108583738}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/time}{18694}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/einspect}{4721}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/@1}{10}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/@3}{17}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/@5}{17}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/@10}{30}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/exam}{0.13859315361752955}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/javaexam}{0.002165689078908047}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/outputlength}{160.63333333333333}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/dev/distance}{13.945892432317322}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/time}{20210}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/einspect}{7768}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/@1}{3}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/@3}{7}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/@5}{10}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/@10}{10}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/exam}{0.25533442158903913}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/javaexam}{7.84488638762666e-05}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/outputlength}{2.1}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/dev/distance}{23.4528805986718}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/time}{1}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/einspect}{8279}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/@3}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/@5}{10}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/@10}{13}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/exam}{0.20856706862705324}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/javaexam}{0.00278045955163677}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/outputlength}{12.433333333333334}
\pgfkeyssetvalue{/flpy/stmt/st/favg/dev/distance}{7.661867443102397}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/time}{38}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/einspect}{2081}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/@1}{20}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/@3}{33}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/@5}{37}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/@10}{47}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/exam}{0.05815756343511883}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/javaexam}{0.005338259423315434}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/outputlength}{1431.4666666666665}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/dev/distance}{9.193634913967903}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/time}{18694}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/einspect}{4720}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/@3}{25}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/@5}{28}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/@10}{40}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/exam}{0.14005571570917544}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/javaexam}{0.004474997644664697}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/outputlength}{160.63333333333333}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/dev/distance}{23.17590675907735}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/time}{521}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/einspect}{526}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/@5}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/@10}{57}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/exam}{0.008854186103602725}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/javaexam}{0.004213188676947862}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/outputlength}{2396.175675675676}
\pgfkeyssetvalue{/flpy/stmt/sbfl/tarantula/mut/distance}{9.56423176802314}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/time}{521}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/einspect}{522}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/@5}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/@10}{57}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/exam}{0.00882554716841561}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/javaexam}{0.0041841574275801015}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/outputlength}{2396.175675675676}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/mut/distance}{9.939073970576185}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/time}{521}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/einspect}{522}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/@1}{11}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/@3}{34}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/@5}{49}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/@10}{57}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/exam}{0.008822822631741587}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/javaexam}{0.004181395568485886}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/outputlength}{2396.175675675676}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/mut/distance}{10.45163519498624}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/time}{17744}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/einspect}{482}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/@1}{18}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/@3}{46}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/@5}{54}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/@10}{68}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/exam}{0.007928819574336011}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/javaexam}{0.003470449924030685}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/outputlength}{138.6891891891892}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/mut/distance}{18.397460537354096}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/time}{17744}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/einspect}{496}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/@1}{11}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/@5}{46}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/@10}{58}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/exam}{0.006798313990211014}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/javaexam}{0.0023244579620409615}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/outputlength}{138.6891891891892}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/mut/distance}{27.049774881803454}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/time}{12932}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/einspect}{10081}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/@1}{5}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/@3}{9}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/@5}{12}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/@10}{12}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/exam}{0.2043890182994061}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/javaexam}{0.00010556862466765817}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/outputlength}{1.135135135135135}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/mut/distance}{12.612974953312067}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/time}{2}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/einspect}{9304}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/@1}{0}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/@3}{4}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/@5}{5}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/@10}{19}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/exam}{0.17048376746971602}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/javaexam}{0.0007175107088746468}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/outputlength}{35.270270270270274}
\pgfkeyssetvalue{/flpy/stmt/st/favg/mut/distance}{8.629261601376617}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/time}{521}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/einspect}{524}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/@3}{35}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/@5}{50}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/@10}{57}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/exam}{0.008834185301253307}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/javaexam}{0.004192913891004616}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/outputlength}{2396.175675675676}
\pgfkeyssetvalue{/flpy/stmt/sbfl/favg/mut/distance}{9.984980311195187}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/time}{17744}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/einspect}{489}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/@1}{14}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/@3}{41}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/@5}{50}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/@10}{63}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/exam}{0.007363566782273513}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/javaexam}{0.0028974539430358234}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/outputlength}{138.6891891891892}
\pgfkeyssetvalue{/flpy/stmt/mbfl/favg/mut/distance}{22.723617709578775}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/time}{-1}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/@1}{70}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/@3}{89}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/@10}{99}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/exam}{0.03858549430871499}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/javaexam}{0.03384424394177811}
\pgfkeyssetvalue{/flpy/mod/avfl/alfa/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/time}{-1}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/@1}{64}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/@3}{87}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/exam}{0.04098960206373947}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/javaexam}{0.03626629279945203}
\pgfkeyssetvalue{/flpy/mod/avfl/sbst/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/time}{-1}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/@1}{67}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/@3}{88}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/exam}{0.039787548186227234}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/javaexam}{0.03505526837061507}
\pgfkeyssetvalue{/flpy/mod/avfl/favg/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@1/java}{4}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@3/java}{23}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@5/java}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/@10/java}{44}
\pgfkeyssetvalue{/flpy/stmt/sbfl/ochiai/all/javaexam/java}{0.033}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@1/java}{5}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@3/java}{24}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@5/java}{31}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/@10/java}{43}
\pgfkeyssetvalue{/flpy/stmt/sbfl/dstar/all/javaexam/java}{0.033}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@1/java}{6}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@3/java}{22}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@5/java}{29}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/@10/java}{36}
\pgfkeyssetvalue{/flpy/stmt/mbfl/metallaxis/all/javaexam/java}{0.118}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@1/java}{7}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@3/java}{12}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@5/java}{16}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/@10/java}{19}
\pgfkeyssetvalue{/flpy/stmt/mbfl/muse/all/javaexam/java}{0.304}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@1/java}{1}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@3/java}{4}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@5/java}{6}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/@10/java}{6}
\pgfkeyssetvalue{/flpy/stmt/ps/favg/all/javaexam/java}{0.331}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@1/java}{6}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@3/java}{9}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@5/java}{11}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/@10/java}{11}
\pgfkeyssetvalue{/flpy/stmt/st/favg/all/javaexam/java}{0.311}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/time}{591}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@10}{56}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/javaexam}{0.003933670244659881}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/einspect}{1584}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/exam}{0.051843632951264776}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@1}{12}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@5}{41}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@3}{32}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/@10}{99}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/javaexam}{0.033990342493138946}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/exam}{0.03873051064858431}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/@1}{70}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/@3}{89}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/@10}{79}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/javaexam}{0.015366033282319778}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/einspect}{67}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/exam}{0.07423039067992367}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/@1}{44}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/@5}{73}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/@3}{64}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/@10}{84}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/javaexam}{0.012833193698378412}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/einspect}{66}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/exam}{0.07188516884294091}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/@1}{53}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/@5}{77}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/@3}{70}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@10/java}{52}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/javaexam/java}{0.018620908434973688}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@1/java}{19}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@5/java}{42}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@3/java}{33}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@10/java}{40}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/javaexam/java}{0.02646145339076598}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@1/java}{10}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@5/java}{30}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/@3/java}{23}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/javaexam}{0.03620025132540632}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/exam}{0.040924049785797854}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/@1}{64}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/@3}{87}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/time}{26116}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@10}{60}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/javaexam}{0.0033443617631956917}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/einspect}{1580}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/exam}{0.05131980318996325}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@1}{20}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@5}{49}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/@3}{39}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@10}{58}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/javaexam}{0.003639016003927786}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/einspect}{1582}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/exam}{0.05158171807061401}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@1}{16}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@5}{45}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@3}{35}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/@10}{98}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/javaexam}{0.035095296909272634}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/einspect}{2}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/exam}{0.03982728021719108}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/@1}{67}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/@5}{93}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/@3}{88}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/@10}{81}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/javaexam}{0.014099613490349095}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/einspect}{66}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/exam}{0.0730577797614323}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/@1}{49}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/@5}{75}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/@3}{67}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@10/java}{46}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/javaexam/java}{0.022541180912869836}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@1/java}{14}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@5/java}{36}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/@3/java}{28}
\pgfkeyssetvalue{/flpy/stmt/comb/alfa/all/outputlength}{2548.362962962963}
\pgfkeyssetvalue{/flpy/stmt/comb/sbst/all/outputlength}{2548.362962962963}
\pgfkeyssetvalue{/flpy/stmt/comb/favg/all/outputlength}{2548.362962962963}
\pgfkeyssetvalue{/flpy/func/comb/alfa/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/comb/sbst/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/comb/favg/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/mod/comb/alfa/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/comb/sbst/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/comb/favg/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/einspect}{1577.5}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/@1}{19.0}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/@3}{37.5}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/@5}{48.0}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/@10}{59.5}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/javaexam}{0.003323445305082064}
\pgfkeyssetvalue{/flpy/stmt/alfafl/favg/all/outputlength}{2548.362962962963}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/einspect}{1584.5}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/@1}{12.0}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/@3}{32.5}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/@5}{42.5}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/@10}{56.0}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/javaexam}{0.003946030935481276}
\pgfkeyssetvalue{/flpy/stmt/sbstfl/favg/all/outputlength}{2548.3481481481485}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/einspect}{66.0}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/@1}{53.0}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/@3}{70.5}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/@5}{76.5}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/@10}{84.0}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/javaexam}{0.012919761855964022}
\pgfkeyssetvalue{/flpy/func/alfafl/favg/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/einspect}{66.5}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/@1}{44.0}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/@3}{64.0}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/@5}{73.0}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/@10}{79.0}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/javaexam}{0.015317222329690433}
\pgfkeyssetvalue{/flpy/func/sbstfl/favg/all/outputlength}{296.34814814814814}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/einspect}{2.0}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/@1}{70.0}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/@3}{89.0}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/@5}{93.0}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/@10}{99.0}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/javaexam}{0.033917293217458525}
\pgfkeyssetvalue{/flpy/mod/alfafl/favg/all/outputlength}{20.918518518518518}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/einspect}{2.0}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/@1}{64.0}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/@3}{87.0}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/@5}{93.0}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/@10}{98.0}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/javaexam}{0.03623327206242918}
\pgfkeyssetvalue{/flpy/mod/sbstfl/favg/all/outputlength}{20.918518518518518}


==> figs/stats.tex <==
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:PS/corrTau}{0.0748108683990909}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:PS/WilcoxonP}{7.44970812013263e-20}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:PS/CliffD}{-0.697997256515775}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:ST/corrTau}{-0.00551600728116301}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:ST/WilcoxonP}{4.69632453473045e-14}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:ST/CliffD}{-0.453772290809328}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:SBFL/corrTau}{0.540395240400838}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:SBFL/WilcoxonP}{0.00520931038798318}
\pgfkeyssetvalue{/flpy/statement/einspect/MBFL:SBFL/CliffD}{0.176186556927298}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:ST/corrTau}{0.146485617820881}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:ST/WilcoxonP}{0.0116745886019255}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:ST/CliffD}{0.183539094650206}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:SBFL/corrTau}{0.0570253731815212}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:SBFL/WilcoxonP}{9.17718332925928e-21}
\pgfkeyssetvalue{/flpy/statement/einspect/PS:SBFL/CliffD}{0.783758573388203}
\pgfkeyssetvalue{/flpy/statement/einspect/ST:SBFL/corrTau}{0.0667513688819089}
\pgfkeyssetvalue{/flpy/statement/einspect/ST:SBFL/WilcoxonP}{3.57426094089792e-17}
\pgfkeyssetvalue{/flpy/statement/einspect/ST:SBFL/CliffD}{0.562194787379973}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:PS/corrTau}{0.561967938087341}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:PS/WilcoxonP}{5.76724770171956e-08}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:PS/CliffD}{0.336954732510288}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:ST/corrTau}{0.179878385848535}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:ST/WilcoxonP}{6.78946425811962e-24}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:ST/CliffD}{0.998353909465021}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:SBFL/corrTau}{0.592482034273079}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:SBFL/WilcoxonP}{7.54381658530857e-23}
\pgfkeyssetvalue{/flpy/statement/time/MBFL:SBFL/CliffD}{0.766913580246914}
\pgfkeyssetvalue{/flpy/statement/time/PS:ST/corrTau}{0.085461580983969}
\pgfkeyssetvalue{/flpy/statement/time/PS:ST/WilcoxonP}{7.42416508740563e-24}
\pgfkeyssetvalue{/flpy/statement/time/PS:ST/CliffD}{0.96323731138546}
\pgfkeyssetvalue{/flpy/statement/time/PS:SBFL/corrTau}{0.324267551133223}
\pgfkeyssetvalue{/flpy/statement/time/PS:SBFL/WilcoxonP}{1.96521841180797e-14}
\pgfkeyssetvalue{/flpy/statement/time/PS:SBFL/CliffD}{0.485432098765432}
\pgfkeyssetvalue{/flpy/statement/time/ST:SBFL/corrTau}{0.200884466556108}
\pgfkeyssetvalue{/flpy/statement/time/ST:SBFL/WilcoxonP}{8.48796405900451e-24}
\pgfkeyssetvalue{/flpy/statement/time/ST:SBFL/CliffD}{-0.864362139917696}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Ochiai/corrTau}{0.993881655156452}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Ochiai/WilcoxonP}{1}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Ochiai/CliffD}{0.00219478737997256}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Tarantula/corrTau}{0.936853579376171}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Tarantula/WilcoxonP}{0.0908887852457271}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/DStar:Tarantula/CliffD}{-0.0205761316872428}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/Ochiai:Tarantula/corrTau}{0.943224617816058}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/Ochiai:Tarantula/WilcoxonP}{0.0584752615656529}
\pgfkeyssetvalue{/flpy/statement-intra-SBFL/einspect/Ochiai:Tarantula/CliffD}{-0.0227709190672154}
\pgfkeyssetvalue{/flpy/statement-intra-MBFL/einspect/Metallaxis:Muse/corrTau}{0.615555642276624}
\pgfkeyssetvalue{/flpy/statement-intra-MBFL/einspect/Metallaxis:Muse/WilcoxonP}{0.00366191684658065}
\pgfkeyssetvalue{/flpy/statement-intra-MBFL/einspect/Metallaxis:Muse/CliffD}{-0.10803840877915}
\pgfkeyssetvalue{/flpy/m6/mutability/mbfl/significant}{0.87}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 50:MBFL}{-2.5262775}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 50:PS}{1.117685}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 50:ST}{1.2182375}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 50:SBFL}{-2.88013}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 70:MBFL}{-2.7709055}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 70:PS}{0.94775795}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 70:ST}{1.0616545}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 70:SBFL}{-3.1258475}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 90:MBFL}{-3.2180915}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 90:PS}{0.6775959}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 90:ST}{0.7788652}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 90:SBFL}{-3.5455925}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 95:MBFL}{-3.51031975}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 95:PS}{0.535925525}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 95:ST}{0.644767625}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 95:SBFL}{-3.76600675}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 99:MBFL}{-4.0641862}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 99:PS}{0.232960895}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 99:ST}{0.33158403}
\pgfkeyssetvalue{/flpy/m2/einspect/family/lower 99:SBFL}{-4.2131177}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 99:MBFL}{-0.702209474999999}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 99:PS}{2.59205895}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 99:ST}{2.70007475}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 99:SBFL}{-0.978632644999998}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 95:MBFL}{-1.0036095}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 95:PS}{2.30851975}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 95:ST}{2.4006195}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 95:SBFL}{-1.33387875}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 90:MBFL}{-1.1621255}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 90:PS}{2.153348}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 90:ST}{2.257362}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 90:SBFL}{-1.514786}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 70:MBFL}{-1.4888745}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 70:PS}{1.862479}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 70:ST}{1.977887}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 70:SBFL}{-1.837451}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 50:MBFL}{-1.6824225}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 50:PS}{1.703535}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 50:ST}{1.810125}
\pgfkeyssetvalue{/flpy/m2/einspect/family/upper 50:SBFL}{-2.0364775}
\pgfkeyssetvalue{/flpy/m2/einspect/family/MBFL}{-2.1329160825}
\pgfkeyssetvalue{/flpy/m2/einspect/family/PS}{1.411442171875}
\pgfkeyssetvalue{/flpy/m2/einspect/family/ST}{1.5187468519}
\pgfkeyssetvalue{/flpy/m2/einspect/family/SBFL}{-2.4731523275}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 50:CL}{0.8576515}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 50:DEV}{-1.5181075}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 50:DS}{0.1622345}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 50:WEB}{-1.3309425}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 70:CL}{0.73787805}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 70:DEV}{-1.6876235}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 70:DS}{0.04688615}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 70:WEB}{-1.5082515}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 90:CL}{0.53094055}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 90:DEV}{-2.0290295}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 90:DS}{-0.1804682}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 90:WEB}{-1.894603}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 95:CL}{0.40753025}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 95:DEV}{-2.22066825}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 95:DS}{-0.31008255}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 95:WEB}{-2.123565}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 99:CL}{0.17324546}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 99:DEV}{-2.64810525}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 99:DS}{-0.55104856}
\pgfkeyssetvalue{/flpy/m2/einspect/category/lower 99:WEB}{-2.5519435}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 99:CL}{2.07250355}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 99:DEV}{-0.177008155}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 99:DS}{1.3620486}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 99:WEB}{0.0438689545000003}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 95:CL}{1.7999425}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 95:DEV}{-0.40564255}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 95:DS}{1.12326375}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 95:WEB}{-0.193428325}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 90:CL}{1.6730295}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 90:DEV}{-0.52403775}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 90:DS}{0.99301}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 90:WEB}{-0.31669545}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 70:CL}{1.4488815}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 70:DEV}{-0.7515989}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 70:DS}{0.7566167}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 70:WEB}{-0.5624215}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 50:CL}{1.3150325}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 50:DEV}{-0.9015535}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 50:DS}{0.621022}
\pgfkeyssetvalue{/flpy/m2/einspect/category/upper 50:WEB}{-0.70125675}
\pgfkeyssetvalue{/flpy/m2/einspect/category/CL}{1.089910848175}
\pgfkeyssetvalue{/flpy/m2/einspect/category/DEV}{-1.225378347225}
\pgfkeyssetvalue{/flpy/m2/einspect/category/DS}{0.393016353284575}
\pgfkeyssetvalue{/flpy/m2/einspect/category/WEB}{-1.04013070633775}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 50:MBFL}{1.5663375}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 50:PS}{0.87735675}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 50:ST}{-2.946875}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 50:SBFL}{-2.48673}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 70:MBFL}{1.407346}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 70:PS}{0.7103954}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 70:ST}{-3.2094265}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 70:SBFL}{-2.733209}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 90:MBFL}{1.1276775}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 90:PS}{0.425159}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 90:ST}{-3.6871695}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 90:SBFL}{-3.182601}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 95:MBFL}{0.967736825}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 95:PS}{0.245108975}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 95:ST}{-3.92562525}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 95:SBFL}{-3.45412175}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 99:MBFL}{0.626437305}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 99:PS}{-0.0473359034999997}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 99:ST}{-4.3522941}
\pgfkeyssetvalue{/flpy/m2/time/family/lower 99:SBFL}{-4.0203258}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 99:MBFL}{2.97825215}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 99:PS}{2.31325605}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 99:ST}{-1.0736534}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 99:SBFL}{-0.523117094999996}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 95:MBFL}{2.70623925}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 95:PS}{2.0606435}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 95:ST}{-1.43820975}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 95:SBFL}{-0.86405605}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 90:MBFL}{2.578099}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 90:PS}{1.9228}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 90:ST}{-1.5988785}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 90:SBFL}{-1.037878}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 70:MBFL}{2.3357665}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 70:PS}{1.6489455}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 70:ST}{-1.9309575}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 70:SBFL}{-1.40563}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 50:MBFL}{2.17211}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 50:PS}{1.4788225}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 50:ST}{-2.12484}
\pgfkeyssetvalue{/flpy/m2/time/family/upper 50:SBFL}{-1.63189}
\pgfkeyssetvalue{/flpy/m2/time/family/MBFL}{1.8625292902}
\pgfkeyssetvalue{/flpy/m2/time/family/PS}{1.1746280953275}
\pgfkeyssetvalue{/flpy/m2/time/family/ST}{-2.564445435}
\pgfkeyssetvalue{/flpy/m2/time/family/SBFL}{-2.06971550775}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 50:CL}{-0.8226835}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 50:DEV}{0.035917725}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 50:DS}{0.22997525}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 50:WEB}{-0.23261775}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 70:CL}{-0.91694215}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 70:DEV}{-0.0503907649999998}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 70:DS}{0.15723225}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 70:WEB}{-0.32312575}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 90:CL}{-1.097481}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 90:DEV}{-0.19879025}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 90:DS}{0.0213224}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 90:WEB}{-0.4800993}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 95:CL}{-1.193378}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 95:DEV}{-0.2838526}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 95:DS}{-0.0632587875}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 95:WEB}{-0.578146275}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 99:CL}{-1.46282195}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 99:DEV}{-0.487885135}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 99:DS}{-0.22869648}
\pgfkeyssetvalue{/flpy/m2/time/category/lower 99:WEB}{-0.7566351}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 99:CL}{-0.110575348999999}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 99:DEV}{0.738491820000001}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 99:DS}{0.903944345}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 99:WEB}{0.51016309}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 95:CL}{-0.215460325}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 95:DEV}{0.599098075}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 95:DS}{0.769458525}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 95:WEB}{0.3571841}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 90:CL}{-0.2763427}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 90:DEV}{0.52126265}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 90:DS}{0.71423625}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 90:WEB}{0.282513849999999}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 70:CL}{-0.4095806}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 70:DEV}{0.39238235}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 70:DS}{0.5725315}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 70:WEB}{0.1460154}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 50:CL}{-0.494305}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 50:DEV}{0.31617325}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 50:DS}{0.49809975}
\pgfkeyssetvalue{/flpy/m2/time/category/upper 50:WEB}{0.068308625}
\pgfkeyssetvalue{/flpy/m2/time/category/CL}{-0.663901802125}
\pgfkeyssetvalue{/flpy/m2/time/category/DEV}{0.172121719109}
\pgfkeyssetvalue{/flpy/m2/time/category/DS}{0.3640750835075}
\pgfkeyssetvalue{/flpy/m2/time/category/WEB}{-0.08639932358645}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 50:logmutability MBFL}{-0.7547445}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 50:logmutability PS}{0.3759405}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 50:logmutability ST}{0.26624775}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 50:logmutability SBFL}{-0.515623}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 70:logmutability MBFL}{-0.8841669}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 70:logmutability PS}{0.25446255}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 70:logmutability ST}{0.147502}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 70:logmutability SBFL}{-0.76394705}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 80:logmutability MBFL}{-0.9720413}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 80:logmutability PS}{0.1822384}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 80:logmutability ST}{0.07889756}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 80:logmutability SBFL}{-0.9411668}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 87:logmutability MBFL}{-1.05968925}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 87:logmutability PS}{0.115193315}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 87:logmutability ST}{0.0086214319}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 87:logmutability SBFL}{-1.11161255}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 90:logmutability MBFL}{-1.1205065}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 90:logmutability PS}{0.085546755}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 90:logmutability ST}{-0.027511595}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 90:logmutability SBFL}{-1.225794}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 95:logmutability MBFL}{-1.28001225}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 95:logmutability PS}{-0.00431204149999994}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 95:logmutability ST}{-0.130285675}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 95:logmutability SBFL}{-1.45534775}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 99:logmutability MBFL}{-1.4713408}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 99:logmutability PS}{-0.178970675}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 99:logmutability ST}{-0.261238665}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/lower 99:logmutability SBFL}{-1.8345544}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 99:logmutability MBFL}{0.25625661}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 99:logmutability PS}{1.56417885}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 99:logmutability ST}{1.4698448}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 99:logmutability SBFL}{1.3301171}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 95:logmutability MBFL}{0.1087532}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 95:logmutability PS}{1.3620565}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 95:logmutability ST}{1.25861325}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 95:logmutability SBFL}{0.992993675}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 90:logmutability MBFL}{0.0151696599999999}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 90:logmutability PS}{1.221132}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 90:logmutability ST}{1.1073075}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 90:logmutability SBFL}{0.84015345}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 87:logmutability MBFL}{-0.0229480944999999}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 87:logmutability PS}{1.16346775}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 87:logmutability ST}{1.0500677}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 87:logmutability SBFL}{0.76403437}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 80:logmutability MBFL}{-0.0932349600000002}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 80:logmutability PS}{1.068632}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 80:logmutability ST}{0.955611}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 80:logmutability SBFL}{0.6521943}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 70:logmutability MBFL}{-0.16356845}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 70:logmutability PS}{0.9829318}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 70:logmutability ST}{0.87455715}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 70:logmutability SBFL}{0.52767515}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 50:logmutability MBFL}{-0.27993625}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 50:logmutability PS}{0.85509625}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 50:logmutability ST}{0.749353}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/upper 50:logmutability SBFL}{0.331809}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/logmutability MBFL}{-0.5291964366535}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/logmutability PS}{0.625550630091}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/logmutability ST}{0.51708127530175}
\pgfkeyssetvalue{/flpy/m6/einspect/logmutability/logmutability SBFL}{-0.109275289464}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 50:crashing MBFL}{-1.5439225}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 50:crashing PS}{0.6979465}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 50:crashing ST}{-2.229575}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 50:crashing SBFL}{-0.557907}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 70:crashing MBFL}{-1.743097}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 70:crashing PS}{0.50589745}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 70:crashing ST}{-2.479337}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 70:crashing SBFL}{-0.87455075}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 80:crashing MBFL}{-1.874443}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 80:crashing PS}{0.3868135}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 80:crashing ST}{-2.653464}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 80:crashing SBFL}{-1.070707}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 87:crashing MBFL}{-2.00333665}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 87:crashing PS}{0.248499565}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 87:crashing ST}{-2.8226749}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 87:crashing SBFL}{-1.3077794}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 90:crashing MBFL}{-2.074271}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 90:crashing PS}{0.1867658}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 90:crashing ST}{-2.9160775}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 90:crashing SBFL}{-1.4007575}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 95:crashing MBFL}{-2.25423675}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 95:crashing PS}{0.0457672750000002}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 95:crashing ST}{-3.157148}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 95:crashing SBFL}{-1.6832555}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 99:crashing MBFL}{-2.5844665}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 99:crashing PS}{-0.22599418}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 99:crashing ST}{-3.72883035}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/lower 99:crashing SBFL}{-2.2694496}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 99:crashing MBFL}{0.107556140000001}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 99:crashing PS}{2.48447375}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 99:crashing ST}{-0.172546394999999}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 99:crashing SBFL}{2.1516732}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 95:crashing MBFL}{-0.190584025}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 95:crashing PS}{2.14954175}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 95:crashing ST}{-0.4905315}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 95:crashing SBFL}{1.60724175}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 90:crashing MBFL}{-0.343026500000002}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 90:crashing PS}{1.952465}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 90:crashing ST}{-0.7176368}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 90:crashing SBFL}{1.340869}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 87:crashing MBFL}{-0.399429795}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 87:crashing PS}{1.8871615}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 87:crashing ST}{-0.81324367}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 87:crashing SBFL}{1.25926105}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 80:crashing MBFL}{-0.5205948}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 80:crashing PS}{1.768569}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 80:crashing ST}{-0.953928}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 80:crashing SBFL}{1.075584}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 70:crashing MBFL}{-0.6415296}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 70:crashing PS}{1.627476}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 70:crashing ST}{-1.105512}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 70:crashing SBFL}{0.8747363}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 50:crashing MBFL}{-0.83476175}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 50:crashing PS}{1.41554}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 50:crashing ST}{-1.3252025}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/upper 50:crashing SBFL}{0.581589}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/crashing MBFL}{-1.1932547987975}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/crashing PS}{1.0644355637525}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/crashing ST}{-1.7871074044125}
\pgfkeyssetvalue{/flpy/m6/einspect/crashing/crashing SBFL}{0.00502130608705}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 50:predicate MBFL}{-0.59165975}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 50:predicate PS}{-0.286226}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 50:predicate ST}{0.23657575}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 50:predicate SBFL}{-0.637463}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 70:predicate MBFL}{-0.7619661}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 70:predicate PS}{-0.4756684}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 70:predicate ST}{0.054673455}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 70:predicate SBFL}{-0.95892545}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 80:predicate MBFL}{-0.9020018}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 80:predicate PS}{-0.5995323}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 80:predicate ST}{-0.06710679}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 80:predicate SBFL}{-1.167584}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 87:predicate MBFL}{-1.01068645}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 87:predicate PS}{-0.71890176}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 87:predicate ST}{-0.183570605}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 87:predicate SBFL}{-1.3752713}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 90:predicate MBFL}{-1.071021}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 90:predicate PS}{-0.777294}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 90:predicate ST}{-0.2229248}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 90:predicate SBFL}{-1.4714315}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 95:predicate MBFL}{-1.21743375}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 95:predicate PS}{-0.935833725}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 95:predicate ST}{-0.375249225}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 95:predicate SBFL}{-1.776968}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 99:predicate MBFL}{-1.54477605}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 99:predicate PS}{-1.1746152}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 99:predicate ST}{-0.651481505}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/lower 99:predicate SBFL}{-2.28115135}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 99:predicate MBFL}{0.973989965000001}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 99:predicate PS}{1.32411835}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 99:predicate ST}{1.8931751}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 99:predicate SBFL}{2.06602095}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 95:predicate MBFL}{0.694470375000001}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 95:predicate PS}{1.03394625}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 95:predicate ST}{1.5518615}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 95:predicate SBFL}{1.53690225}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 90:predicate MBFL}{0.55932135}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 90:predicate PS}{0.8917026}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 90:predicate ST}{1.399975}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 90:predicate SBFL}{1.302487}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 87:predicate MBFL}{0.493542565}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 87:predicate PS}{0.83245287}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 87:predicate ST}{1.3270633}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 87:predicate SBFL}{1.19595145}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 80:predicate MBFL}{0.3862723}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 80:predicate PS}{0.7108285}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 80:predicate ST}{1.221673}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 80:predicate SBFL}{0.9985885}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 70:predicate MBFL}{0.2497229}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 70:predicate PS}{0.5776847}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 70:predicate ST}{1.105351}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 70:predicate SBFL}{0.81038855}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 50:predicate MBFL}{0.0721588}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 50:predicate PS}{0.39488575}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 50:predicate ST}{0.919414}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/upper 50:predicate SBFL}{0.49630225}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/predicate MBFL}{-0.2579525699835}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/predicate PS}{0.055023161026325}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/predicate ST}{0.58027280242025}
\pgfkeyssetvalue{/flpy/m6/einspect/predicate/predicate SBFL}{-0.07751487353475}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/CL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/CL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/CL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/CL:coef.delta}{-2.3152891954}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/CL:outcome.delta}{-159.299830699841}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/CL:ratio.delta}{0.0987376254057489}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/CL:coef.delta}{-0.696894494890425}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/CL:outcome.delta}{-88.7064991797041}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/CL:ratio.delta}{0.498129849044942}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/CL:coef.delta}{-2.13004155451275}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/CL:outcome.delta}{-155.748049074124}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/CL:ratio.delta}{0.118832355729168}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DEV:coef.delta}{2.3152891954}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DEV:outcome.delta}{159.299830699841}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DEV:ratio.delta}{10.1278514233114}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DEV:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DEV:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DEV:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DEV:coef.delta}{1.61839470050957}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DEV:outcome.delta}{70.5933315201374}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DEV:ratio.delta}{5.04498510064369}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DEV:coef.delta}{0.18524764088725}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DEV:outcome.delta}{3.55178162571792}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DEV:ratio.delta}{1.2035164431071}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DS:coef.delta}{0.696894494890425}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DS:outcome.delta}{88.7064991797041}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/DS:ratio.delta}{2.00750868858248}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DS:coef.delta}{-1.61839470050957}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DS:outcome.delta}{-70.5933315201374}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/DS:ratio.delta}{0.198216640892043}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/DS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DS:coef.delta}{-1.43314705962233}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DS:outcome.delta}{-67.0415498944194}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/DS:ratio.delta}{0.23855698661103}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/WEB:coef.delta}{2.13004155451275}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/WEB:outcome.delta}{155.748049074124}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/CL/WEB:ratio.delta}{8.41521649439574}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/WEB:coef.delta}{-0.18524764088725}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/WEB:outcome.delta}{-3.55178162571792}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DEV/WEB:ratio.delta}{0.830898493931926}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/WEB:coef.delta}{1.43314705962233}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/WEB:outcome.delta}{67.0415498944194}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/DS/WEB:ratio.delta}{4.19187052203385}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/WEB:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/WEB:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/category/WEB/WEB:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/MBFL:coef.delta}{3.544358254375}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/MBFL:outcome.delta}{236.740767910714}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/MBFL:ratio.delta}{34.6174626071753}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/MBFL:coef.delta}{-0.340236245}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/MBFL:outcome.delta}{-2.03095396348916}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/MBFL:ratio.delta}{0.711602190443701}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/MBFL:coef.delta}{3.6516629344}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/MBFL:outcome.delta}{264.354891888454}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/MBFL:ratio.delta}{38.5387001222087}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/PS:coef.delta}{-3.544358254375}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/PS:outcome.delta}{-236.740767910714}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/PS:ratio.delta}{0.0288871547677422}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/PS:coef.delta}{-3.884594499375}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/PS:outcome.delta}{-238.771721874203}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/PS:ratio.delta}{0.0205561626084115}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/PS:coef.delta}{0.107304680025}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/PS:outcome.delta}{27.6141239777402}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/PS:ratio.delta}{1.11327339497785}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/SBFL:coef.delta}{0.340236245}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/SBFL:outcome.delta}{2.03095396348916}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/SBFL:ratio.delta}{1.40527954161647}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/SBFL:coef.delta}{3.884594499375}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/SBFL:outcome.delta}{238.771721874203}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/SBFL:ratio.delta}{48.6472119845366}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/SBFL:coef.delta}{3.9918991794}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/SBFL:outcome.delta}{266.385845851943}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/SBFL:ratio.delta}{54.1576468422321}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/ST:coef.delta}{-3.6516629344}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/ST:outcome.delta}{-264.354891888454}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/MBFL/ST:ratio.delta}{0.0259479431539968}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/ST:coef.delta}{-0.107304680025}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/ST:outcome.delta}{-27.6141239777402}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/PS/ST:ratio.delta}{0.898251951866593}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/ST:coef.delta}{-3.9918991794}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/ST:outcome.delta}{-266.385845851943}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/SBFL/ST:ratio.delta}{0.0184646131858927}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/einspect/family/ST/ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/CL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/CL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/CL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/CL:coef.delta}{0.836023521234}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/CL:outcome.delta}{4404.28925690882}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/CL:ratio.delta}{2.30717428207451}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/CL:coef.delta}{1.0279768856325}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/CL:outcome.delta}{11118.0965964186}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/CL:ratio.delta}{2.79540468667046}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/CL:coef.delta}{0.57750247853855}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/CL:outcome.delta}{1444.1427878494}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/CL:ratio.delta}{1.78158332711254}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DEV:coef.delta}{-0.836023521234}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DEV:outcome.delta}{-4404.28925690882}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DEV:ratio.delta}{0.433430628873361}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DEV:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DEV:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DEV:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DEV:coef.delta}{0.1919533643985}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DEV:outcome.delta}{6713.80733950981}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DEV:ratio.delta}{1.21161401129912}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DEV:coef.delta}{-0.25852104269545}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DEV:outcome.delta}{-2960.14646905942}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DEV:ratio.delta}{0.772192781860685}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DS:coef.delta}{-1.0279768856325}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DS:outcome.delta}{-11118.0965964186}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/DS:ratio.delta}{0.357729957586597}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DS:coef.delta}{-0.1919533643985}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DS:outcome.delta}{-6713.80733950981}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/DS:ratio.delta}{0.825345358071402}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/DS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DS:coef.delta}{-0.45047440709395}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DS:outcome.delta}{-9673.95380856923}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/DS:ratio.delta}{0.637325728044959}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/WEB:coef.delta}{-0.57750247853855}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/WEB:outcome.delta}{-1444.1427878494}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/CL/WEB:ratio.delta}{0.561298472421565}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/WEB:coef.delta}{0.25852104269545}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/WEB:outcome.delta}{2960.14646905942}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DEV/WEB:ratio.delta}{1.29501340013874}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/WEB:coef.delta}{0.45047440709395}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/WEB:outcome.delta}{9673.95380856923}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/DS/WEB:ratio.delta}{1.56905638042822}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/WEB:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/WEB:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/category/WEB/WEB:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/MBFL:coef.delta}{-0.6879011948725}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/MBFL:outcome.delta}{-341812618709.654}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/MBFL:ratio.delta}{0.50262988498193}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/MBFL:coef.delta}{-3.93224479795}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/MBFL:outcome.delta}{-341818237478.079}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/MBFL:ratio.delta}{0.0195996259335646}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/MBFL:coef.delta}{-4.4269747252}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/MBFL:outcome.delta}{-341818237497.854}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/MBFL:ratio.delta}{0.0119505888555931}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/PS:coef.delta}{0.6879011948725}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/PS:outcome.delta}{341812618709.654}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/PS:ratio.delta}{1.98953550093018}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/PS:coef.delta}{-3.2443436030775}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/PS:outcome.delta}{-5618768.42415353}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/PS:ratio.delta}{0.0389941515997786}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/PS:coef.delta}{-3.7390735303275}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/PS:outcome.delta}{-5618788.19925456}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/PS:ratio.delta}{0.023776120785223}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/SBFL:coef.delta}{3.93224479795}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/SBFL:outcome.delta}{341818237478.079}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/SBFL:ratio.delta}{51.0213819074723}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/SBFL:coef.delta}{3.2443436030775}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/SBFL:outcome.delta}{5618768.42415353}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/SBFL:ratio.delta}{25.6448713197719}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/SBFL:coef.delta}{-0.49472992725}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/SBFL:outcome.delta}{-19.7751010302638}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/SBFL:ratio.delta}{0.609735558020399}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/ST:coef.delta}{4.4269747252}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/ST:outcome.delta}{341818237497.854}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/MBFL/ST:ratio.delta}{83.6778850049703}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/ST:coef.delta}{3.7390735303275}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/ST:outcome.delta}{5618788.19925456}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/PS/ST:ratio.delta}{42.0590057155794}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/ST:coef.delta}{0.49472992725}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/ST:outcome.delta}{19.7751010302638}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/SBFL/ST:ratio.delta}{1.64005524500926}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m2/time/family/ST/ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/MBFL:coef.delta}{1.26812964375}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/MBFL:outcome.delta}{17.691932576341}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/MBFL:ratio.delta}{3.55419872397402}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/MBFL:coef.delta}{-2.0025586375}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/MBFL:outcome.delta}{-5.9915887305987}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/MBFL:ratio.delta}{0.134989451923003}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/MBFL:coef.delta}{-0.444935924999999}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/MBFL:outcome.delta}{-2.48758491702068}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/MBFL:ratio.delta}{0.64086533816332}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/PS:coef.delta}{-1.26812964375}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/PS:outcome.delta}{-17.691932576341}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/PS:ratio.delta}{0.281357368470911}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/PS:coef.delta}{-3.27068828125}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/PS:outcome.delta}{-23.6835213069397}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/PS:ratio.delta}{0.0379802769643868}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/PS:coef.delta}{-1.71306556875}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/PS:outcome.delta}{-20.1795174933617}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/PS:ratio.delta}{0.180312185089852}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/SBFL:coef.delta}{2.0025586375}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/SBFL:outcome.delta}{5.9915887305987}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/SBFL:ratio.delta}{7.40798622228936}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/SBFL:coef.delta}{3.27068828125}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/SBFL:outcome.delta}{23.6835213069397}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/SBFL:ratio.delta}{26.3294551784779}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/SBFL:coef.delta}{1.5576227125}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/SBFL:outcome.delta}{3.50400381357802}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/SBFL:ratio.delta}{4.74752159545668}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/ST:coef.delta}{0.444935924999999}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/ST:outcome.delta}{2.48758491702068}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/MBFL/ST:ratio.delta}{1.56039021062668}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/ST:coef.delta}{1.71306556875}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/ST:outcome.delta}{20.1795174933617}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/PS/ST:ratio.delta}{5.54593689551089}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/ST:coef.delta}{-1.5576227125}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/ST:outcome.delta}{-3.50400381357802}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/SBFL/ST:ratio.delta}{0.210636219318515}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m3/einspect/family/ST/ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing MBFL:coef.delta}{2.15683540262}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing MBFL:outcome.delta}{143.705228253692}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing MBFL:ratio.delta}{8.64374037250212}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing MBFL:coef.delta}{1.1803868772335}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing MBFL:outcome.delta}{42.4067681429403}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing MBFL:ratio.delta}{3.25563348975706}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing MBFL:coef.delta}{-0.67235787205}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing MBFL:outcome.delta}{-9.20272133254542}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing MBFL:ratio.delta}{0.510503455753343}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing PS:coef.delta}{-2.15683540262}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing PS:outcome.delta}{-143.705228253692}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing PS:ratio.delta}{0.11569065669548}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing PS:coef.delta}{-0.9764485253865}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing PS:outcome.delta}{-101.298460110752}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing PS:ratio.delta}{0.37664637638979}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing PS:coef.delta}{-2.82919327467}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing PS:outcome.delta}{-152.907949586238}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing PS:ratio.delta}{0.059060480041416}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing SBFL:coef.delta}{-1.1803868772335}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing SBFL:outcome.delta}{-42.4067681429403}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing SBFL:ratio.delta}{0.307159882445681}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing SBFL:coef.delta}{0.9764485253865}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing SBFL:outcome.delta}{101.298460110752}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing SBFL:ratio.delta}{2.65501027670874}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing SBFL:coef.delta}{-1.8527447492835}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing SBFL:outcome.delta}{-51.6094894754857}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing SBFL:ratio.delta}{0.15680618145731}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing ST:coef.delta}{0.67235787205}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing ST:outcome.delta}{9.20272133254542}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing MBFL/crashing ST:ratio.delta}{1.95885059881586}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing ST:coef.delta}{2.82919327467}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing ST:outcome.delta}{152.907949586238}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing PS/crashing ST:ratio.delta}{16.9317960046846}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing ST:coef.delta}{1.8527447492835}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing ST:outcome.delta}{51.6094894754857}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing SBFL/crashing ST:ratio.delta}{6.37729961093558}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/crashing/crashing ST/crashing ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable MBFL:coef.delta}{1.2555643154823}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable MBFL:outcome.delta}{116.316100292253}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable MBFL:ratio.delta}{3.50981846049072}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable MBFL:coef.delta}{-0.04124731340195}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable MBFL:outcome.delta}{-1.87269582786142}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable MBFL:ratio.delta}{0.959591780691417}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable MBFL:coef.delta}{1.1185544808608}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable MBFL:outcome.delta}{95.4893148666807}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable MBFL:ratio.delta}{3.0604270983866}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable PS:coef.delta}{-1.2555643154823}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable PS:outcome.delta}{-116.316100292253}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable PS:ratio.delta}{0.284915020892615}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable PS:coef.delta}{-1.29681162888425}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable PS:outcome.delta}{-118.188796120114}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable PS:ratio.delta}{0.273402112244077}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable PS:coef.delta}{-0.1370098346215}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable PS:outcome.delta}{-20.8267854255721}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable PS:ratio.delta}{0.871961650677144}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable SBFL:coef.delta}{0.04124731340195}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable SBFL:outcome.delta}{1.87269582786142}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable SBFL:ratio.delta}{1.04210980139854}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable SBFL:coef.delta}{1.29681162888425}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable SBFL:outcome.delta}{118.188796120114}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable SBFL:ratio.delta}{3.6576162188069}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable SBFL:coef.delta}{1.15980179426275}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable SBFL:outcome.delta}{97.3620106945421}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable SBFL:ratio.delta}{3.18930107569436}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable ST:coef.delta}{-1.1185544808608}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable ST:outcome.delta}{-95.4893148666807}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable MBFL/ismutable ST:ratio.delta}{0.326751779360201}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable ST:coef.delta}{0.1370098346215}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable ST:outcome.delta}{20.8267854255721}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable PS/ismutable ST:ratio.delta}{1.14683942719663}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable ST:coef.delta}{-1.15980179426275}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable ST:outcome.delta}{-97.3620106945421}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable SBFL/ismutable ST:ratio.delta}{0.313548321800345}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/mutable/ismutable ST/ismutable ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate MBFL:coef.delta}{0.39294543644445}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate MBFL:outcome.delta}{18.0006348893976}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate MBFL:ratio.delta}{1.48133756007987}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate MBFL:coef.delta}{0.43850001253675}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate MBFL:outcome.delta}{20.5826199020843}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate MBFL:ratio.delta}{1.55037992304284}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate MBFL:coef.delta}{0.94674469269725}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate MBFL:outcome.delta}{58.9866924010772}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate MBFL:ratio.delta}{2.57730606534059}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate PS:coef.delta}{-0.39294543644445}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate PS:outcome.delta}{-18.0006348893976}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate PS:ratio.delta}{0.67506558055956}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate PS:coef.delta}{0.0455545760923}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate PS:outcome.delta}{2.58198501268673}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate PS:ratio.delta}{1.0466081228368}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate PS:coef.delta}{0.5537992562528}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate PS:outcome.delta}{40.9860575116796}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate PS:ratio.delta}{1.73985061527882}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate SBFL:coef.delta}{-0.43850001253675}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate SBFL:outcome.delta}{-20.5826199020843}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate SBFL:ratio.delta}{0.645003192531902}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate SBFL:coef.delta}{-0.0455545760923}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate SBFL:outcome.delta}{-2.58198501268673}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate SBFL:ratio.delta}{0.955467455468936}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate SBFL:coef.delta}{0.5082446801605}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate SBFL:outcome.delta}{38.4040724989929}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate SBFL:ratio.delta}{1.66237064027652}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate ST:coef.delta}{-0.94674469269725}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate ST:outcome.delta}{-58.9866924010772}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate MBFL/predicate ST:ratio.delta}{0.388002035710046}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate ST:coef.delta}{-0.5537992562528}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate ST:outcome.delta}{-40.9860575116796}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate PS/predicate ST:ratio.delta}{0.574761988884743}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate ST:coef.delta}{-0.5082446801605}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate ST:outcome.delta}{-38.4040724989929}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate SBFL/predicate ST:ratio.delta}{0.601550566264609}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m4/einspect/predicate/predicate ST/predicate ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/CL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/CL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/CL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/CL:coef.delta}{-2.46104017479625}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/CL:outcome.delta}{-127.292291497055}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/CL:ratio.delta}{0.085346129887339}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/CL:coef.delta}{-0.31623790102325}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/CL:outcome.delta}{-37.7309056784644}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/CL:ratio.delta}{0.728886026808034}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/CL:coef.delta}{-2.33572496300125}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/CL:outcome.delta}{-125.706562599304}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/CL:ratio.delta}{0.0967403239427568}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DEV:coef.delta}{2.46104017479625}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DEV:outcome.delta}{127.292291497055}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DEV:ratio.delta}{11.7169929242257}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DEV:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DEV:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DEV:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DEV:coef.delta}{2.144802273773}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DEV:outcome.delta}{89.5613858185908}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DEV:ratio.delta}{8.54035241867673}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DEV:coef.delta}{0.125315211795}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DEV:outcome.delta}{1.58572889775118}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DEV:ratio.delta}{1.13350569112459}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DS:coef.delta}{0.31623790102325}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DS:outcome.delta}{37.7309056784644}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/DS:ratio.delta}{1.37195660668546}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DS:coef.delta}{-2.144802273773}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DS:outcome.delta}{-89.5613858185908}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/DS:ratio.delta}{0.11709118675397}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/DS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DS:coef.delta}{-2.019487061978}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DS:outcome.delta}{-87.9756569208396}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/DS:ratio.delta}{0.132723526566157}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/WEB:coef.delta}{2.33572496300125}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/WEB:outcome.delta}{125.706562599304}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/CL/WEB:ratio.delta}{10.3369511207314}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/WEB:coef.delta}{-0.125315211795}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/WEB:outcome.delta}{-1.58572889775118}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DEV/WEB:ratio.delta}{0.882218772989017}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/WEB:coef.delta}{2.019487061978}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/WEB:outcome.delta}{87.9756569208396}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/DS/WEB:ratio.delta}{7.53445923169877}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/WEB:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/WEB:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/category/WEB/WEB:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing MBFL:coef.delta}{2.25769036255}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing MBFL:outcome.delta}{154.28417324165}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing MBFL:ratio.delta}{9.56098124560721}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing MBFL:coef.delta}{1.19827610488455}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing MBFL:outcome.delta}{41.7095915736318}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing MBFL:ratio.delta}{3.31439831994265}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing MBFL:coef.delta}{-0.593852605615}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing MBFL:outcome.delta}{-8.07023171987616}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing MBFL:ratio.delta}{0.552195788867669}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing PS:coef.delta}{-2.25769036255}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing PS:outcome.delta}{-154.28417324165}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing PS:ratio.delta}{0.104591775081606}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing PS:coef.delta}{-1.05941425766545}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing PS:outcome.delta}{-112.574581668018}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing PS:ratio.delta}{0.346658803610294}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing PS:coef.delta}{-2.851542968165}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing PS:outcome.delta}{-162.354404961526}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing PS:ratio.delta}{0.0577551377502572}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing SBFL:coef.delta}{-1.19827610488455}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing SBFL:outcome.delta}{-41.7095915736318}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing SBFL:ratio.delta}{0.301713886946848}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing SBFL:coef.delta}{1.05941425766545}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing SBFL:outcome.delta}{112.574581668018}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing SBFL:ratio.delta}{2.88468081463807}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing SBFL:coef.delta}{-1.79212871049955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing SBFL:outcome.delta}{-49.779823293508}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing SBFL:ratio.delta}{0.166605137814946}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing ST:coef.delta}{0.593852605615}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing ST:outcome.delta}{8.07023171987616}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing MBFL/crashing ST:ratio.delta}{1.81095187641796}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing ST:coef.delta}{2.851542968165}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing ST:outcome.delta}{162.354404961526}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing PS/crashing ST:ratio.delta}{17.3144769271293}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing ST:coef.delta}{1.79212871049955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing ST:outcome.delta}{49.779823293508}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing SBFL/crashing ST:ratio.delta}{6.00221585669667}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/crashing/crashing ST/crashing ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/MBFL:coef.delta}{1.00344464824718}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/MBFL:outcome.delta}{48.7130426307368}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/MBFL:ratio.delta}{2.72766149875258}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/MBFL:coef.delta}{0.07872333934125}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/MBFL:outcome.delta}{2.30938748896576}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/MBFL:ratio.delta}{1.08190496012241}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/MBFL:coef.delta}{1.0592698107795}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/MBFL:outcome.delta}{53.1286021962154}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/MBFL:ratio.delta}{2.88426416157028}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/PS:coef.delta}{-1.00344464824718}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/PS:outcome.delta}{-48.7130426307368}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/PS:ratio.delta}{0.366614405950784}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/PS:coef.delta}{-0.924721308905925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/PS:outcome.delta}{-46.403655141771}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/PS:ratio.delta}{0.396641944250486}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/PS:coef.delta}{0.055825162532325}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/PS:outcome.delta}{4.41555956547859}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/PS:ratio.delta}{1.05741279219922}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/SBFL:coef.delta}{-0.07872333934125}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/SBFL:outcome.delta}{-2.30938748896576}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/SBFL:ratio.delta}{0.924295605306082}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/SBFL:coef.delta}{0.924721308905925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/SBFL:outcome.delta}{46.403655141771}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/SBFL:ratio.delta}{2.52116553605961}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/SBFL:coef.delta}{0.98054647143825}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/SBFL:outcome.delta}{50.8192147072496}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/SBFL:ratio.delta}{2.66591268908124}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/ST:coef.delta}{-1.0592698107795}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/ST:outcome.delta}{-53.1286021962154}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/MBFL/ST:ratio.delta}{0.346708881011638}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/ST:coef.delta}{-0.055825162532325}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/ST:outcome.delta}{-4.41555956547859}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/PS/ST:ratio.delta}{0.945704466011032}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/ST:coef.delta}{-0.98054647143825}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/ST:outcome.delta}{-50.8192147072496}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/SBFL/ST:ratio.delta}{0.375106058084983}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/family/ST/ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability MBFL:coef.delta}{1.1547470667445}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability MBFL:outcome.delta}{76.0849129074274}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability MBFL:ratio.delta}{3.17322070297245}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability MBFL:coef.delta}{0.4199211471895}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability MBFL:outcome.delta}{18.2697822004949}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability MBFL:ratio.delta}{1.52184154940398}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability MBFL:coef.delta}{1.04627771195525}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability MBFL:outcome.delta}{64.665044105586}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability MBFL:ratio.delta}{2.84703388991987}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability PS:coef.delta}{-1.1547470667445}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability PS:outcome.delta}{-76.0849129074274}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability PS:ratio.delta}{0.315137235510681}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability PS:coef.delta}{-0.734825919555}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability PS:outcome.delta}{-57.8151307069324}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability PS:ratio.delta}{0.479588938764461}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability PS:coef.delta}{-0.10846935478925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability PS:outcome.delta}{-11.4198688018414}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability PS:ratio.delta}{0.897206389474571}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability SBFL:coef.delta}{-0.4199211471895}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability SBFL:outcome.delta}{-18.2697822004949}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability SBFL:ratio.delta}{0.657098631846165}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability SBFL:coef.delta}{0.734825919555}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability SBFL:outcome.delta}{57.8151307069324}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability SBFL:ratio.delta}{2.08511898246912}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability SBFL:coef.delta}{0.62635656476575}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability SBFL:outcome.delta}{46.395261905091}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability SBFL:ratio.delta}{1.87078207388601}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability ST:coef.delta}{-1.04627771195525}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability ST:outcome.delta}{-64.665044105586}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability MBFL/logmutability ST:ratio.delta}{0.351242745490516}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability ST:coef.delta}{0.10846935478925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability ST:outcome.delta}{11.4198688018414}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability PS/logmutability ST:ratio.delta}{1.11457075175939}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability ST:coef.delta}{-0.62635656476575}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability ST:outcome.delta}{-46.395261905091}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability SBFL/logmutability ST:ratio.delta}{0.534535804014193}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/logmutability/logmutability ST/logmutability ST:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate MBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate MBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate MBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate MBFL:coef.delta}{0.312975731009825}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate MBFL:outcome.delta}{16.8747752096196}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate MBFL:ratio.delta}{1.36748834306373}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate MBFL:coef.delta}{0.18043769644875}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate MBFL:outcome.delta}{9.08013367503642}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate MBFL:ratio.delta}{1.19774149560713}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate MBFL:coef.delta}{0.83822537240375}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate MBFL:outcome.delta}{60.257942312032}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate MBFL:ratio.delta}{2.31225993333523}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate PS:coef.delta}{-0.312975731009825}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate PS:outcome.delta}{-16.8747752096196}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate PS:ratio.delta}{0.731267659481175}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate PS:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate PS:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate PS:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate PS:coef.delta}{-0.132538034561075}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate PS:outcome.delta}{-7.79464153458316}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate PS:ratio.delta}{0.875869620156105}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate PS:coef.delta}{0.525249641393925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate PS:outcome.delta}{43.3831671024124}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate PS:ratio.delta}{1.69088090956215}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate SBFL:coef.delta}{-0.18043769644875}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate SBFL:outcome.delta}{-9.08013367503642}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate SBFL:ratio.delta}{0.834904696604092}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate SBFL:coef.delta}{0.132538034561075}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate SBFL:outcome.delta}{7.79464153458316}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate SBFL:ratio.delta}{1.14172244017525}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate SBFL:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate SBFL:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate SBFL:ratio.delta}{1}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate SBFL:coef.delta}{0.657787675955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate SBFL:outcome.delta}{51.1778086369955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate SBFL:ratio.delta}{1.93051667811105}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate ST:coef.delta}{-0.83822537240375}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate ST:outcome.delta}{-60.257942312032}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate MBFL/predicate ST:ratio.delta}{0.4324773290335}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate ST:coef.delta}{-0.525249641393925}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate ST:outcome.delta}{-43.3831671024124}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate PS/predicate ST:ratio.delta}{0.591407706092646}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate ST:coef.delta}{-0.657787675955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate ST:outcome.delta}{-51.1778086369955}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate SBFL/predicate ST:ratio.delta}{0.517996042892759}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate ST:coef.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate ST:outcome.delta}{0}
\pgfkeyssetvalue{/flpy/deltas/m6/einspect/predicate/predicate ST/predicate ST:ratio.delta}{1}
\pgfkeyssetvalue{}{}


==> stats-discussion.tex <==
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/dstar/pval}{2.79690539361965e-06}
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/dstar/cohend}{-0.273513849984438}
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/ochiai/pval}{1.44410933105894e-06}
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/ochiai/cohend}{-0.281315489158626}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/dstar/pval}{4.80227415794797e-28}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/dstar/cohend}{-0.641103848946986}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/ochiai/pval}{5.0343356159017e-28}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/ochiai/cohend}{-0.640854860462704}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/dstar/pval}{0.0203315101206638}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/dstar/cohend}{0.111297852474323}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/ochiai/pval}{0.0134696328365303}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/ochiai/cohend}{0.11870525988173}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/dstar/pval}{0.0346377109968765}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/dstar/cohend}{0.106567071272954}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/ochiai/pval}{0.0397409905158073}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/ochiai/cohend}{0.103765950824774}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/e_inspect/pval}{0.361310428526179}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/e_inspect/cohend}{0.00674897119341565}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/e_inspect/pval}{0.0865712192909329}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/e_inspect/cohend}{-0.00126200274348421}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/e_inspect/pval}{0.361310428526179}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/e_inspect/cohend}{-0.00674897119341563}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/e_inspect/pval}{0.0407602539105694}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/e_inspect/cohend}{-0.00801097393689985}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/e_inspect/pval}{0.0865712192909329}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/e_inspect/cohend}{0.00126200274348423}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/e_inspect/pval}{0.0407602539105694}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/e_inspect/cohend}{0.00801097393689988}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/exam/pval}{0.583882420770365}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/exam/cohend}{0.00241426611796983}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/exam/pval}{0.0934924836898357}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/exam/cohend}{-0.00949245541838134}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/exam/pval}{0.583882420770365}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/exam/cohend}{-0.00241426611796982}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/exam/pval}{0.0559296803251122}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/exam/cohend}{-0.0119067215363512}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/exam/pval}{0.0934924836898357}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/exam/cohend}{0.00949245541838135}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/exam/pval}{0.0559296803251122}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/exam/cohend}{0.0119067215363512}
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/dstar/esmagnitude}{s}
\pgfkeyssetvalue{/flpy/discussion/python/e_inspect/dstar/mean}{85.1922751322751}
\pgfkeyssetvalue{/flpy/discussion/java/e_inspect/dstar/mean}{177.061174756479}
\pgfkeyssetvalue{/flpy/discussion/python/java/e_inspect/ochiai/esmagnitude}{s}
\pgfkeyssetvalue{/flpy/discussion/python/e_inspect/ochiai/mean}{85.5330158730159}
\pgfkeyssetvalue{/flpy/discussion/java/e_inspect/ochiai/mean}{177.985777931082}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/dstar/esmagnitude}{l}
\pgfkeyssetvalue{/flpy/discussion/python/exam/dstar/mean}{-0.107418467292241}
\pgfkeyssetvalue{/flpy/discussion/java/exam/dstar/mean}{0.000987470636658941}
\pgfkeyssetvalue{/flpy/discussion/python/java/exam/ochiai/esmagnitude}{l}
\pgfkeyssetvalue{/flpy/discussion/python/exam/ochiai/mean}{-0.107416973842509}
\pgfkeyssetvalue{/flpy/discussion/java/exam/ochiai/mean}{0.000935287809059463}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/dstar/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/python/@5/dstar/mean}{0.422222222222222}
\pgfkeyssetvalue{/flpy/discussion/java/@5/dstar/mean}{0.310924369747899}
\pgfkeyssetvalue{/flpy/discussion/python/java/@5/ochiai/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/python/@5/ochiai/mean}{0.42962962962963}
\pgfkeyssetvalue{/flpy/discussion/java/@5/ochiai/mean}{0.310924369747899}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/dstar/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/python/@10/dstar/mean}{0.540740740740741}
\pgfkeyssetvalue{/flpy/discussion/java/@10/dstar/mean}{0.434173669467787}
\pgfkeyssetvalue{/flpy/discussion/python/java/@10/ochiai/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/python/@10/ochiai/mean}{0.540740740740741}
\pgfkeyssetvalue{/flpy/discussion/java/@10/ochiai/mean}{0.436974789915966}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/e_inspect/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/dstar/ochiai/exam/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/dstar/tarantula/exam/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/ochiai/dstar/exam/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/ochiai/tarantula/exam/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/tarantula/dstar/exam/esmagnitude}{n}
\pgfkeyssetvalue{/flpy/discussion/tarantula/ochiai/exam/esmagnitude}{n}


==> stats-extra.tex <==
\pgfkeyssetvalue{/flpy/num extra tests threshold}{50}
\pgfkeyssetvalue{/flpy/max extra tests}{642}
\pgfkeyssetvalue{/flpy/zero transitive delta}{0.481481481481481}
\pgfkeyssetvalue{/flpy/10percent transitive delta}{0.696296296296296}
\pgfkeyssetvalue{/flpy/perc more than threshold transitive delta}{0.296296296296296}
\pgfkeyssetvalue{/flpy/num more than threshold transitive delta}{40}
\pgfkeyssetvalue{/flpy/projects more than threshold transitive delta}{7}
\pgfkeyssetvalue{/flpy/extra tests new experiments}{35}
\pgfkeyssetvalue{/flpy/extra experiments no change}{20}
\pgfkeyssetvalue{/flpy/extra experiments top-1 change}{0}
\pgfkeyssetvalue{/flpy/extra experiments top-3 change}{0}
\pgfkeyssetvalue{/flpy/extra experiments top-5 change}{0}
\pgfkeyssetvalue{/flpy/extra experiments top-10 change}{-1}
\pgfkeyssetvalue{/flpy/extra experiments top-10 change einspect nontransitive}{13.3333333333333}
\pgfkeyssetvalue{/flpy/extra experiments top-10 change einspect transitive}{9.33333333333333}


==> table-macros.tex <==
% The number of decimal points for exam scores in tables
\newcommand{\examdec}{4}
\newcommand{\examdecjava}{4}
\newcommand{\cddec}{1}


==> test-data.tex <==
\pgfkeyssetvalue{/flpy/test/all/max/n}{1036}
\pgfkeyssetvalue{/flpy/test/all/max/p}{100.0}
\pgfkeyssetvalue{/flpy/test/all/mean/n}{86.64444444444445}
\pgfkeyssetvalue{/flpy/test/all/mean/p}{4.5918127002072735}
\pgfkeyssetvalue{/flpy/test/all/median/n}{53}
\pgfkeyssetvalue{/flpy/test/all/median/p}{8.938740293356341}
\pgfkeyssetvalue{/flpy/test/all/min/n}{1}
\pgfkeyssetvalue{/flpy/test/all/min/p}{0.008731336767659128}
\pgfkeyssetvalue{/flpy/test/black/max/n}{129}
\pgfkeyssetvalue{/flpy/test/black/max/p}{93.47826086956522}
\pgfkeyssetvalue{/flpy/test/black/mean/n}{83.3076923076923}
\pgfkeyssetvalue{/flpy/test/black/mean/p}{91.23841617523168}
\pgfkeyssetvalue{/flpy/test/black/median/n}{91}
\pgfkeyssetvalue{/flpy/test/black/median/p}{91.0}
\pgfkeyssetvalue{/flpy/test/black/min/n}{16}
\pgfkeyssetvalue{/flpy/test/black/min/p}{88.46153846153845}
\pgfkeyssetvalue{/flpy/test/cli/max/n}{126}
\pgfkeyssetvalue{/flpy/test/cli/max/p}{100.0}
\pgfkeyssetvalue{/flpy/test/cli/mean/n}{40.55813953488372}
\pgfkeyssetvalue{/flpy/test/cli/mean/p}{17.859703020993344}
\pgfkeyssetvalue{/flpy/test/cli/median/n}{17}
\pgfkeyssetvalue{/flpy/test/cli/median/p}{15.151515151515152}
\pgfkeyssetvalue{/flpy/test/cli/min/n}{1}
\pgfkeyssetvalue{/flpy/test/cli/min/p}{0.6122448979591837}
\pgfkeyssetvalue{/flpy/test/cookiecutter/max/n}{60}
\pgfkeyssetvalue{/flpy/test/cookiecutter/max/p}{28.037383177570092}
\pgfkeyssetvalue{/flpy/test/cookiecutter/mean/n}{39.75}
\pgfkeyssetvalue{/flpy/test/cookiecutter/mean/p}{20.866141732283463}
\pgfkeyssetvalue{/flpy/test/cookiecutter/median/n}{44.0}
\pgfkeyssetvalue{/flpy/test/cookiecutter/median/p}{26.30627608825283}
\pgfkeyssetvalue{/flpy/test/cookiecutter/min/n}{11}
\pgfkeyssetvalue{/flpy/test/cookiecutter/min/p}{5.213270142180095}
\pgfkeyssetvalue{/flpy/test/dev/max/n}{198}
\pgfkeyssetvalue{/flpy/test/dev/max/p}{93.47826086956522}
\pgfkeyssetvalue{/flpy/test/dev/mean/n}{80.76666666666667}
\pgfkeyssetvalue{/flpy/test/dev/mean/p}{19.916159789577513}
\pgfkeyssetvalue{/flpy/test/dev/median/n}{80.0}
\pgfkeyssetvalue{/flpy/test/dev/median/p}{27.584583061653262}
\pgfkeyssetvalue{/flpy/test/dev/min/n}{2}
\pgfkeyssetvalue{/flpy/test/dev/min/p}{0.2242152466367713}
\pgfkeyssetvalue{/flpy/test/ds/max/n}{1036}
\pgfkeyssetvalue{/flpy/test/ds/max/p}{51.61290322580645}
\pgfkeyssetvalue{/flpy/test/ds/mean/n}{112.80952380952381}
\pgfkeyssetvalue{/flpy/test/ds/mean/p}{2.13487854442557}
\pgfkeyssetvalue{/flpy/test/ds/median/n}{67.5}
\pgfkeyssetvalue{/flpy/test/ds/median/p}{3.169367738415564}
\pgfkeyssetvalue{/flpy/test/ds/min/n}{1}
\pgfkeyssetvalue{/flpy/test/ds/min/p}{0.008731336767659128}
\pgfkeyssetvalue{/flpy/test/fastapi/max/n}{282}
\pgfkeyssetvalue{/flpy/test/fastapi/max/p}{49.91150442477876}
\pgfkeyssetvalue{/flpy/test/fastapi/mean/n}{37.61538461538461}
\pgfkeyssetvalue{/flpy/test/fastapi/mean/p}{8.801295896328295}
\pgfkeyssetvalue{/flpy/test/fastapi/median/n}{5}
\pgfkeyssetvalue{/flpy/test/fastapi/median/p}{1.5424164524421593}
\pgfkeyssetvalue{/flpy/test/fastapi/min/n}{1}
\pgfkeyssetvalue{/flpy/test/fastapi/min/p}{0.2506265664160401}
\pgfkeyssetvalue{/flpy/test/httpie/max/n}{17}
\pgfkeyssetvalue{/flpy/test/httpie/max/p}{100.0}
\pgfkeyssetvalue{/flpy/test/httpie/mean/n}{8.0}
\pgfkeyssetvalue{/flpy/test/httpie/mean/p}{7.191011235955057}
\pgfkeyssetvalue{/flpy/test/httpie/median/n}{7.0}
\pgfkeyssetvalue{/flpy/test/httpie/median/p}{4.658247968915577}
\pgfkeyssetvalue{/flpy/test/httpie/min/n}{1}
\pgfkeyssetvalue{/flpy/test/httpie/min/p}{0.7874015748031495}
\pgfkeyssetvalue{/flpy/test/keras/max/n}{288}
\pgfkeyssetvalue{/flpy/test/keras/max/p}{51.61290322580645}
\pgfkeyssetvalue{/flpy/test/keras/mean/n}{76.55555555555556}
\pgfkeyssetvalue{/flpy/test/keras/mean/p}{13.945956886954761}
\pgfkeyssetvalue{/flpy/test/keras/median/n}{58.0}
\pgfkeyssetvalue{/flpy/test/keras/median/p}{10.51003654604828}
\pgfkeyssetvalue{/flpy/test/keras/min/n}{18}
\pgfkeyssetvalue{/flpy/test/keras/min/p}{3.0100334448160537}
\pgfkeyssetvalue{/flpy/test/luigi/max/n}{198}
\pgfkeyssetvalue{/flpy/test/luigi/max/p}{33.22147651006711}
\pgfkeyssetvalue{/flpy/test/luigi/mean/n}{90.84615384615384}
\pgfkeyssetvalue{/flpy/test/luigi/mean/p}{11.559166095722814}
\pgfkeyssetvalue{/flpy/test/luigi/median/n}{91}
\pgfkeyssetvalue{/flpy/test/luigi/median/p}{11.303744798890431}
\pgfkeyssetvalue{/flpy/test/luigi/min/n}{2}
\pgfkeyssetvalue{/flpy/test/luigi/min/p}{0.2242152466367713}
\pgfkeyssetvalue{/flpy/test/pandas/max/n}{1036}
\pgfkeyssetvalue{/flpy/test/pandas/max/p}{8.938740293356341}
\pgfkeyssetvalue{/flpy/test/pandas/mean/n}{159.83333333333334}
\pgfkeyssetvalue{/flpy/test/pandas/mean/p}{1.3935915134781662}
\pgfkeyssetvalue{/flpy/test/pandas/median/n}{91.5}
\pgfkeyssetvalue{/flpy/test/pandas/median/p}{0.7735426408340571}
\pgfkeyssetvalue{/flpy/test/pandas/min/n}{1}
\pgfkeyssetvalue{/flpy/test/pandas/min/p}{0.008731336767659128}
\pgfkeyssetvalue{/flpy/test/sanic/max/n}{298}
\pgfkeyssetvalue{/flpy/test/sanic/max/p}{64.22413793103449}
\pgfkeyssetvalue{/flpy/test/sanic/mean/n}{220.33333333333334}
\pgfkeyssetvalue{/flpy/test/sanic/mean/p}{47.34957020057307}
\pgfkeyssetvalue{/flpy/test/sanic/median/n}{265}
\pgfkeyssetvalue{/flpy/test/sanic/median/p}{56.50319829424307}
\pgfkeyssetvalue{/flpy/test/sanic/min/n}{98}
\pgfkeyssetvalue{/flpy/test/sanic/min/p}{21.166306695464364}
\pgfkeyssetvalue{/flpy/test/spacy/max/n}{152}
\pgfkeyssetvalue{/flpy/test/spacy/max/p}{16.890380313199106}
\pgfkeyssetvalue{/flpy/test/spacy/mean/n}{80.5}
\pgfkeyssetvalue{/flpy/test/spacy/mean/p}{8.614232209737828}
\pgfkeyssetvalue{/flpy/test/spacy/median/n}{75.0}
\pgfkeyssetvalue{/flpy/test/spacy/median/p}{7.8189486028731885}
\pgfkeyssetvalue{/flpy/test/spacy/min/n}{13}
\pgfkeyssetvalue{/flpy/test/spacy/min/p}{1.3713080168776373}
\pgfkeyssetvalue{/flpy/test/thefuck/max/n}{18}
\pgfkeyssetvalue{/flpy/test/thefuck/max/p}{5.426356589147287}
\pgfkeyssetvalue{/flpy/test/thefuck/mean/n}{7.375}
\pgfkeyssetvalue{/flpy/test/thefuck/mean/p}{1.953965888392118}
\pgfkeyssetvalue{/flpy/test/thefuck/median/n}{5.0}
\pgfkeyssetvalue{/flpy/test/thefuck/median/p}{1.7137534627375657}
\pgfkeyssetvalue{/flpy/test/thefuck/min/n}{3}
\pgfkeyssetvalue{/flpy/test/thefuck/min/p}{0.6122448979591837}
\pgfkeyssetvalue{/flpy/test/tornado/max/n}{787}
\pgfkeyssetvalue{/flpy/test/tornado/max/p}{76.7056530214425}
\pgfkeyssetvalue{/flpy/test/tornado/mean/n}{410.5}
\pgfkeyssetvalue{/flpy/test/tornado/mean/p}{41.88775510204082}
\pgfkeyssetvalue{/flpy/test/tornado/median/n}{411.5}
\pgfkeyssetvalue{/flpy/test/tornado/median/p}{40.481153747979235}
\pgfkeyssetvalue{/flpy/test/tornado/min/n}{32}
\pgfkeyssetvalue{/flpy/test/tornado/min/p}{3.361344537815126}
\pgfkeyssetvalue{/flpy/test/tqdm/max/n}{77}
\pgfkeyssetvalue{/flpy/test/tqdm/max/p}{100.0}
\pgfkeyssetvalue{/flpy/test/tqdm/mean/n}{47.857142857142854}
\pgfkeyssetvalue{/flpy/test/tqdm/mean/p}{82.1078431372549}
\pgfkeyssetvalue{/flpy/test/tqdm/median/n}{63}
\pgfkeyssetvalue{/flpy/test/tqdm/median/p}{95.23809523809523}
\pgfkeyssetvalue{/flpy/test/tqdm/min/n}{1}
\pgfkeyssetvalue{/flpy/test/tqdm/min/p}{1.6666666666666667}
\pgfkeyssetvalue{/flpy/test/web/max/n}{787}
\pgfkeyssetvalue{/flpy/test/web/max/p}{76.7056530214425}
\pgfkeyssetvalue{/flpy/test/web/mean/n}{139.6}
\pgfkeyssetvalue{/flpy/test/web/mean/p}{25.680647534952172}
\pgfkeyssetvalue{/flpy/test/web/median/n}{32.0}
\pgfkeyssetvalue{/flpy/test/web/median/p}{4.458177002869124}
\pgfkeyssetvalue{/flpy/test/web/min/n}{1}
\pgfkeyssetvalue{/flpy/test/web/min/p}{0.2506265664160401}
\pgfkeyssetvalue{/flpy/test/youtube-dl/max/n}{126}
\pgfkeyssetvalue{/flpy/test/youtube-dl/max/p}{55.75221238938053}
\pgfkeyssetvalue{/flpy/test/youtube-dl/mean/n}{78.6875}
\pgfkeyssetvalue{/flpy/test/youtube-dl/mean/p}{43.82178907065785}
\pgfkeyssetvalue{/flpy/test/youtube-dl/median/n}{89.5}
\pgfkeyssetvalue{/flpy/test/youtube-dl/median/p}{51.03860539674058}
\pgfkeyssetvalue{/flpy/test/youtube-dl/min/n}{15}
\pgfkeyssetvalue{/flpy/test/youtube-dl/min/p}{14.285714285714285}
